Contrastive Learning Augmented Social Recommendations

Recommender systems are essential for modern content platforms, yet traditional behavior-based models often struggle with cold users who have limited interaction data. Engaging these users is crucial for platform growth. To bridge this gap, we propose leveraging the social-relation graph to enrich interest representations from behavior-based models. However, extracting value from social graphs is challenging due to relation noise and cross-domain inconsistency. To address the noise propagation and obtain accurate social interest, we employ a dual-view denoising strategy, employing low-rank SVD to the user-item interaction matrix for a denoised social graph and contrastive learning to align the original and reconstructed social graphs. Addressing the interest inconsistency between social and behavioral interests, we adopt a "mutual distillation" technique to isolate the original interests into aligned social/behavior interests and social/behavior specific interests, maximizing the utility of both. Experimental results on widely adopted industry datasets verify the method's effectiveness, particularly for cold users, offering a fresh perspective for future research. The implementation can be accessed at https://github.com/WANGLin0126/CLSRec.

==> sections/3-relatedworks.tex <==
\section{Related Work}

Social recommender systems enhance user behavior information by leveraging social information, 
such as friend connections and trust data, to provide more accurate recommendations. 
This approach aims to mitigate inherent issues like data sparsity in the behavioral domain~\cite{yang2016social,wu2019neural,xiao2023incorporating}. 
Social recommendation algorithms have evolved from traditional collaborative filtering models~\cite{ma2008sorec,jamali2010matrix} 
and probabilistic generative models~\cite{ye2012exploring,yang2012bayesian} to recent methods based on graph neural networks (GNNs)~\cite{fan2019graph,wu2020diffnet++,liao2022sociallgn}.

In recent years, graph neural networks have demonstrated powerful capabilities in handling graph-structured data, 
making them a popular research direction in social recommender systems. 
In particular, some studies have enhanced the performance of GNNs by incorporating social relationships. 
For example, they improve social recommendation effectiveness by integrating implicit social relationships 
between users\cite{dai2024gnnes} or enhance the performance of GNN-based social recommendation models by combining heterogeneous relationships~\cite{liao2022sociallgn,wang2023hrgnn}. 
Additionally, some research focuses on addressing specific issues in social recommender systems, 
such as data sparsity and the cold start problem. 
For instance, by constructing influence neighborhoods among users to enhance the social-based recommendation process\cite{gulati2019little} 
or by integrating trust and social reputation to improve recommendation accuracy in social e-commerce\cite{hu2021gnneco}.

It is noteworthy that despite the progress made in existing studies, 
several challenges and unresolved issues remain. 
Effectively utilizing social information to improve the accuracy of recommender systems is still an open question. 
Addressing the sparsity and noise issues in social data is a key focus of current research~\cite{li2023survey,sharma2024survey}.
